Mask Reference Image Quality Assessment

Understanding semantic information is an essential step in knowing what is being learned in both full-reference (FR) and no-reference (NR) image quality assessment (IQA) methods. However, especially for many severely distorted images, even if there is an undistorted image as a reference (FR-IQA), it is difficult to perceive the lost semantic and texture information of distorted images directly. In this paper, we propose a Mask Reference IQA (MR-IQA) method that masks specific patches of a distorted image and supplements missing patches with the reference image patches. In this way, our model only needs to input the reconstructed image for quality assessment. First, we design a mask generator to select the best candidate patches from reference images and supplement the lost semantic information in distorted images, thus providing more reference for quality assessment; in addition, the different masked patches imply different data augmentations, which favors model training and reduces overfitting. Second, we provide a Mask Reference Network (MRNet): the dedicated modules can prevent disturbances due to masked patches and help eliminate the patch discontinuity in the reconstructed image. Our method achieves state-of-the-art performances on the benchmark KADID-10k, LIVE and CSIQ datasets and has better generalization performance across datasets. The code and results are available in the supplementary material.

==> table/table4.tex <==
% \begin{table}[]
% \scriptsize
% \begin{center}
% \setlength{\tabcolsep}{2mm}{
% \begin{tabular}{l|cc|cc|cc}
% \Xhline{1.2pt} \hline \specialrule{0em}{1pt}{1pt}


% \multicolumn{1}{c|}{Trained on:}  & \multicolumn{2}{c|}{TID2013} & \multicolumn{2}{c}{LIVE} \\ \hline \specialrule{0em}{1pt}{1pt}
% \multicolumn{1}{c|}{Tested on:}    & LIVE           & CSIQ   & CSIQ          & TID2013       \\ \hline \specialrule{0em}{1pt}{1pt}
% \rowcolor[HTML]{EFEFEF} 
% DOG-SSIMc\cite{pei2015image}              & \uline{0.948}    & -           & -             & -             \\ \specialrule{0em}{1pt}{1pt}
% WaDIQaM\cite{bosse2017deep}             & 0.936          & -           & -             & -             \\ \specialrule{0em}{1pt}{1pt}
% \rowcolor[HTML]{EFEFEF} 
% DualCNN\cite{varga2020composition}               & -              & -           & 0.751         & \uline{0.729}   \\ \specialrule{0em}{1pt}{1pt}
% DeepFL-IQA\cite{lin2020deepfl}        & 0.780          & 0.698       & \uline{0.894}   & 0.710         \\ \hline \specialrule{0em}{1pt}{1pt}
% Ours                  & -              & -           & -             & -             \\ \Xhline{1.2pt} \hline \specialrule{0em}{1pt}{1pt}
% \end{tabular}
% \caption{DOG-SSIMc\cite{pei2015image},WaDIQaM\cite{bosse2017deep},DualCNN\cite{varga2020composition},DeepFL-IQA\cite{lin2020deepfl},VTAMIQ\cite{chubarau2021vtamiq} on }
% }
% \end{center}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
Trained on:                & Tested on:                 & metric & DOG-SSIMc & WaDIQaM-FR & DualCNN & DeepFL-IQA & VTAMIQ & ours \\ \hline
\multirow{4}{*}{LIVE}      & \multirow{2}{*}{TID2013}   & PLCC   & 0.751     & 0.751      & -       & 0.577      & 0.874  & -    \\ \cline{3-9} 
                           &                            & SRCC   & 0.751     & 0.751      & -       & 0.577      & 0.874  & -    \\ \cline{2-9} 
                           & \multirow{2}{*}{KADID-10k} & PLCC   & -         & -          & -       & 0.689      & 0.899  & -    \\ \cline{3-9} 
                           &                            & SRCC   & -         & -          & -       & 0.689      & 0.899  & -    \\ \hline
\multirow{4}{*}{TID2013}   & \multirow{2}{*}{LIVE}      & PLCC   & 0.948     & 0.936      & -       & 0.78       & 0.957  & -    \\ \cline{3-9} 
                           &                            & SRCC   & 0.948     & 0.936      & -       & 0.78       & 0.957  & -    \\ \cline{2-9} 
                           & \multirow{2}{*}{KADID-10k} & PLCC   & -         & -          & -       & 0.698      & 0.907  & -    \\ \cline{3-9} 
                           &                            & SRCC   & -         & -          & -       & 0.698      & 0.907  & -    \\ \hline
\multirow{4}{*}{KADID-10k} & \multirow{2}{*}{LIVE}      & PLCC   & -         & -          & 0.751   & 0.894      & 0.974  & -    \\ \cline{3-9} 
                           &                            & SRCC   & -         & -          & 0.751   & 0.894      & 0.974  & -    \\ \cline{2-9} 
                           & \multirow{2}{*}{TID2013}   & PLCC   & -         & -          & 0.729   & 0.71       & 0.897  & -    \\ \cline{3-9} 
                           &                            & SRCC   & -         & -          & 0.729   & 0.71       & 0.897  & -    \\ \hline
\end{tabular}
\end{table}




==> temp.tex <==

\section{Introduction}\label{sec:Introduction}

% -------------------------------------
% 数字图像可能因为任意环节导致质量问题  【写法一】
Digital images are subject to a wide variety of distortions during acquisition, processing, compression, storage, transmission and reproduction, any of which may result in a degradation of visual quality.
% 如何发现，评估and improve the quality of the content to an acceptable level for the human viewers has become highly desirable for automatic quality control and enhancement.
Knowing how to assess and improve the quality of the content has become highly desirable in many image processing and computer vision applications. 
%As consumers are more and more accustomed to high fidelity imagery and video, image quality has become a critical evaluation metric in many image processing and computer vision applications.（VTAMIQ）

Directly asking human observers to assess visual quality requires slow and expensive subjective experiments.

Hence, it is urgent to develop effective methods to evaluate the perceptual quality automatically in manners that are consistent with human observers, which is known as Image Quality Assessment (IQA).

% Image and video compression and applications of visual media continue to be in high demand these days. 
% The goal of image quality assessment (IQA) is to enable models to perceive image quality consistent with human subjective perception.
% Image quality assessment (IQA) aims to evaluate the perceptual quality of images in manners that are consistent with human observers, which has become a

% 现有的IQA方法可以根据有无参考信息，划分为NR-IQA、FR，其中NR方法仅基于失真图像完成质量评估，FR需要借助失真图像的参考图像。
Based on how much information is available from the reference image, the IQA methods can be divided into three categories: full-reference IQA (FR-IQA), reduced-reference IQA (RR-IQA) and no-reference (or blind) IQA (NR-IQA/BIQA).

优势：无论是基于手工特征提取还是最近的基于深度学习的方法，FR方法因为能获取充足的参考信息，并获取在严重失真图像中丢失的语义先验信息，相对于NR方法， 性能具有绝对的优势。
% 其中，基于CNNs-based的FR-IQA一类方法，能够充分利用参考图像和原始图像之间的差异信息进行对比，可以更好地对图像的失真情况进行判断，相对于手工方法，在性能上具有绝对的优势。
Among them, the FR-IQA methods, which are based on CNNs models, makes full use of the difference between the reference image and the original image for comparison, and can better judge the distortion of the image. Compared with manual methods, it has an absolute advantage in performance.

%劣势：数据集中图像少
% the annotation process for IQA image datasets requires multiple human annotations for every image, and thus the collection process is extremely labor-intensive and costly.
全参考IQA数据集因为成本太高，难以获取且数量少，很难训练有效的基于学习的全参考模型
Available datasets with reference images are small and difficult to obtain, as the construction process is extremely labor-intensive and costly. As a results, most available IQA datasets are too small to be effective for training models.
% A key issue is how to power these models as they grow larger and deeper, the number of parameters increases dramatically;
% 劣势：计算复杂
全参考方法需要分别提取参考图像与失真图像中的特征（输入两张图像），基于二者特征的差异完成质量评分，而NR方法仅需要一张失真图像就可以完成质量评分，模型计算量少，且在训练过程中摆脱了完整参考图像的依赖
The full-reference method needs to extract the features in the reference image and the distorted image separately (input two images), and complete the quality scoring based on the difference between the two features, which will make the model more complex and have higher computational consumption compared to the NR-IQA method.

In this paper，我们设想将NR和FR的优势结合起来，仅使用部分参考图像融入到失真图像中进行评估，一方面获取了参考信息判断失真情况，而且对于失真严重的图像补充了丢失的语义信息，另一方面减少了完整参考图像的依赖，而且由于只需要对融合图像进行评估，大大精简了模型和计算量。
% In this paper，我们发现对于IQA任务，完整的失真图像与参考图像并非都是必要的，仅利用部分参考图像块与失真图像融合后，也可获得不弱的性能，因此我们提出了一种基于mask图像的self-reference IQA方法：将部分参考图像块与失真图像生成掩码图像后，利用该图像内部的self-reference即可完成有效的图像质量评估
【图例】展示全参考的输入以及mask后的输入

在IQA任务中完成这种设想主要面临三个挑战

1.在仅输入一张图像的限制下，需要保证选择的ref图像部分能够为失真图像的质量评估提供语义及参考信息，同时又不丢失原有失真图像中的失真相关信息（怎么选+怎么融合的问题）

2.如何让模型能够基于融入的ref图像部分作为参考，提取其中的特征来辅助失真图像的质量评估（怎么评估的问题）

3.如何在现有包含参考图像的IQA数据集较小的前提下，让模型具有足够的鲁棒性

在本论文中我们提出了基于掩码合成图像的自参考IQA方法来解决上述问题。

我们设计了掩码生成策略，通过掩码的方式将少量参考图像patch融入到了失真图像中，恢复其中的语义信息并为其质量判断提供参考。得益于图像的空间信息冗余和掩码位置的选择，引入的掩码块并不会干扰原有图像的失真信息。

我们基于Transformer作为我们的backbone设计了网络，借助网络内部自注意力模块完成不同尺度下mask图像内部的自参考：借助不同局部的少量参考图像块对其他区域的图像块的失真情况进行感知

我们针对这种mask融合方法，设计了一种Random-crop-Grid-sample数据增强策略，对不同尺寸图像随机crop后采样到固定尺寸用于mask，，同时解决了不同尺度输入图像质量评估的问题。


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% 数字图像可能因为任意环节导致质量问题  【写法二】
Digital images are subject to a wide variety of distortions during acquisition, processing, compression, storage, transmission and reproduction, any of which may result in a degradation of visual quality.

% 如何发现，评估and improve the quality of the content to an acceptable level for the human viewers has become highly desirable for automatic quality control and enhancement.
Knowing how to discover and assess the quality of the content has become highly desirable for automatic quality control, enhancement and ...etc. 

Hence, it is urgent to develop effective methods to evaluate the perceptual quality of images in manners that are consistent with human observers, which is known as Image quality assessment (IQA).

% Image and video compression and applications of visual media continue to be in high demand these days. 
% The goal of image quality assessment (IQA) is to enable models to perceive image quality consistent with human subjective perception.
% Image quality assessment (IQA) aims to evaluate the perceptual quality of images in manners that are consistent with human observers, which has become a

% 现有的IQA方法可以根据有无参考信息，划分为NR-IQA、FR，其中NR方法仅基于失真图像完成质量评估，FR需要借助失真图像的参考图像。
Based on how much information is available from the reference image, the IQA methods can be divided into three categories: full-reference IQA (FR-IQA) [6, 29, 36], reduced-reference IQA (RR-IQA) [5, 18] and no-reference (or blind) IQA (NR-IQA/BIQA) [20, 31, 37].

% 其中，基于CNNs-based的FR-IQA一类方法，能够充分利用参考图像和原始图像之间的差异信息进行对比，可以更好地对图像的失真情况进行判断，相对于手工方法，在性能上具有绝对的优势。
Among them, the FR-IQA methods, makes full use of the difference between the reference image and the original image for comparison, and can better judge the distortion of the image. Compared with manual methods, it has an absolute advantage in performance.

但对于以CNNs methods为backbone的FR和NR方法，the FR method needs to extract the features in the reference image and the distorted image separately (input two images), and complete the quality scoring based on the difference between the two features, which will make the model more complex and have higher computational consumption compared to the NR method.


% the annotation process for IQA image datasets requires multiple human annotations for every image, and thus the collection process is extremely labor-intensive and costly.
% A key issue is how to power these models as they grow larger and deeper, the number of parameters increases dramatically; 

另外，available datasets with reference images are small and difficult to obtain, as the construction process is extremely labor-intensive and costly. As a results, most available IQA datasets are too small to be effective for training CNNs.

% 同时，为了获取参考信息用于比较失真程度，全参考方法需要分别提取参考图像与失真图像中的特征（输入两张图像），比较二者特征的差异完成质量评分，相对于NR方法，在模型设计上会更加复杂，同时也会有相对更高的计算消耗。

% 无论是基于数据驱动全参考或是无参考方法，都需要完整的失真或参考图像的输入，

In this paper，我们发现对于IQA任务，完整的失真图像与参考图像并非都是必要的，仅利用部分参考图像块与失真图像进行融合，即可获得不亚于全参考方法的性能。

% 我们提出了基于mask图像的self-reference IQA方法，仅利用部分参考图像块与失真图像生成掩码图像后，利用该图像内部的self-reference即可完成有效的图像质量评估，并获得不亚于全参考方法中借助整张参考图像用于评估的性能。
% 【图例】

这有两方面的advantages：

% 一方面，经过验证我们发现，对于特定结构的模型，得益于图像信息的空间冗余，少量参考图像块的mask不仅不会干扰模型对于原图像质量的判断，而且替代原有失真图像块后，参考图像块的补充了失真图像中由于严重失真丢失的语义信息，这些语义信息对于图像的质量判断是关键的。

（1）仅提取少量参考图像块置于待评测图像中进行比较，能减少“参考图像”信息空间存在大量冗余，不仅不会干扰模型对于原图像质量的判断，同时还能弥补“代评测图像”由于严重失真丢失的语义信息，这些语义信息对于图像的质量判断是关键的[参考文献][]。


% 基于图像内部特征的质量对比，取得了相比较于参考图像作为外部特征进行全参考对比更好的效果；（2）仅利用部分参考图像块作为参考的方法减少了对于完整参考图像的依赖，模型不再需要成对的图像用于训练。Therefore，在不影响失真图像质量判断的前提下,在不同位置mask参考图像块作为一种数据增强手段，可以产生大量的训练样本,一定程度上解决可供全参考训练的数据集较小的问题。
（2）通过替换失真图像的不同位置，可以产生大量的训练样本,能够作为一种数据增强手段，一定程度上解决全参考训练数据缺少的问题，同时，仅利用部分参考图像块作为参考的方法，减少了对于完整参考图像的依赖，使模型不再需要成对的图像用于训练，仅需要完成一张图像的处理,在模型的结构设计上也是更加简洁高效的。

Driven by this analysis, we present a simple and efficient Mask Reference methods for IQA tasks.

同时，为了解决融合后图像仍可能存在的信息空间冗余，我们设计了一种Random-crop-Grid-sample数据增强策略，用于对Mask 图像的进一步采样，同时对不同尺寸图像随机crop后采样到固定尺寸用于mask，同时解决了不同尺度输入图像质量评估的问题。

我们设计了掩码生成策略，通过【什么方式】计算参考图像与失真图像间的统计学差异，从差异最大的的区域中，生成适量参考图像patch，利用掩码的方式融入到了失真图像中，恢复其中的语义信息并为其质量判断提供参考。

% 得益于图像的空间信息冗余和掩码位置的选择，引入的掩码块并不会干扰原有图像的失真信息。





% 我们提出的Mask-IQA相较于全参考IQA，模型从输入层面仅需要完成一张图像的处理,是更加简洁高效的，但是这种将ref与dst图像合并输入模型的策略面临两个主要挑战

% Designing such systems, however, is challenging
% 其一，如何进行mask才不会影响对于待评估图像本身的质量的判断
% 之所以MAE之类的任务Mask位置可以随机，是由于其数据集大，但是IQA里数据量少，关键失真区域一但被mask掉后就会干扰原失真图像的质量判断,而且图像mask后产生的显著边界差异-块效应可能会影响图像质量判断

% 其二，仅输入一张mask image的情况下，如何让模型获取mask position信息，通过mask的refer image patch can be used to 感知图像其他失真区域的失真程度。
% 以解决对Mask位置的鲁棒的问题，否则confuse网络，引入噪声【我们的方法其实是去掉了传统的Transformer中position embedding，改为一个预训练任务来学习position embedding，这块看一下position embedding被提出时的初衷，模仿着写写】

为了解决上述问题，我们设计了mask生成方法，












% 一方面，经过验证我们发现，对于特定结构的模型，得益于图像信息的空间冗余，少量参考图像块的mask不仅不会干扰模型对于原图像质量的判断，而且替代原有失真图像块后，参考图像块的补充了失真图像中由于严重失真丢失的语义信息，这些语义信息对于图像的质量判断是关键的。
（1）仅提取少量参考mask图像块置于待评测图像中进行比较，能减少“参考图像”信息空间的大量冗余，不仅不会干扰模型对于原图像质量的判断，同时还能弥补“代评测图像”由于严重失真丢失的语义信息，这些语义信息对于图像的质量判断是关键的[参考文献]。


% 基于图像内部特征的质量对比，取得了相比较于参考图像作为外部特征进行全参考对比更好的效果；（2）仅利用部分参考图像块作为参考的方法减少了对于完整参考图像的依赖，模型不再需要成对的图像用于训练。Therefore，在不影响失真图像质量判断的前提下,在不同位置mask参考图像块作为一种数据增强手段，可以产生大量的训练样本,一定程度上解决可供全参考训练的数据集较小的问题。
（2）利用不同的mask位置，可以产生大量的训练样本,能够作为一种数据增强手段，一定程度上解决全参考训练数据缺少的问题，同时，仅利用部分参考图像块作为参考的方法，减少了对于完整参考图像的依赖，使模型不再需要成对的图像用于训练，仅需要完成一张图像的处理,是更加简洁高效的。

% 我们提出的Mask-IQA相较于全参考IQA，模型从输入层面仅需要完成一张图像的处理,是更加简洁高效的，但是这种将ref与dst图像合并输入模型的策略面临两个主要挑战

Designing such systems, however, is challenging
其一，如何进行mask才不会影响对于待评估图像本身的质量的判断
之所以MAE之类的任务Mask位置可以随机，是由于其数据集大，但是IQA里数据量少，关键失真区域一但被mask掉后就会干扰原失真图像的质量判断,而且图像mask后产生的显著边界差异-块效应可能会影响图像质量判断

其二，仅输入一张mask image的情况下，如何让模型获取mask position信息，通过mask的refer image patch can be used to 感知图像其他失真区域的失真程度。
% 以解决对Mask位置的鲁棒的问题，否则confuse网络，引入噪声【我们的方法其实是去掉了传统的Transformer中position embedding，改为一个预训练任务来学习position embedding，这块看一下position embedding被提出时的初衷，模仿着写写】

为了解决上述问题，我们设计了mask生成方法，
基于Transformer作为backbone设计了对于maks图像可以实现self-reference的评估模型
%创新点2

此外，为了更好的利用参考和失真图像中的冗余信息，我们设计了一种随机区域的网格采样方法
受限于模型输入尺寸已经被固定，不同输入尺寸的图像只能resize到固定尺寸后在随机区域进行裁剪，但是这样面临的问题是：如果裁剪的位置不恰当，可能输入图像块的质量并不能与整体图像质量保持一致，而且IQA评估过程中语义信息发挥了关键的作用，较小的图像块无法保留原始图像的语义信息，这些问题对于模型的训练造成困扰。
为了解决上述问题，我们基于Crop-Grid-sample的图像预处理策略，由于可以选择性抛弃冗余信息，解决了模型对于不同尺寸图像的质量评估问题，让模型能够对不同长宽比和分辨率的图像都能够有效的进行质量评估
而且在IQA数据集样本有限的前提下，这种基于不同范围随机区域的随机局部抽样产生的训练样本，作为一种数据增强手段一定程度上缓解了模型在训练样本上的过拟合，让模型能够更好的关注于图像的失真情况，训练后在其他数据集上交叉验证时也表现出了更好的鲁棒性。


In general, the main contributions of the proposed method can be summarized into three-folds:%hyper
\begin{itemize}
    % \item 为了评估可能存在的各种不同粒度的复杂失真的图像，我们提取网络中不同层次输出的多尺度特征用于更准确的失真感知
    \item To assess the quality of images with complex distortions of different granularities, we extract multi-scale features from different layers in the network for more comprehensive distortion perception

\end{itemize}

% 我们采用两段式的网络：生成网络用来决定mask块的比重与位置，保证失真图像能够获取足够的参考信息且不影响质量判断，判别网络基于生成网络mask图像中的参考图像块进行质量评估，通过端到端的训练让判别网络获得优于FR-IQA和NR-IQA的性能

% 此外为了解决参考图像较少而产生的数据短缺问题，我们采用了无监督训练策略，通过让网络识别相对于原图像的失真掩码位置，来训练模型获得对于不同类型失真的感知能力   



